Reweighting NNPDFs: the W lepton asymmetry

We present a method for incorporating the information contained in new datasets into an existing set of parton distribution functions without the need for refitting. The method involves reweighting the ensemble of parton densities through the computation of the chi-square to the new dataset. We explain how reweighting may be used to assess the impact of any new data or pseudodata on parton densities and thus on their predictions. We show that the method works by considering the addition of inclusive jet data to a DIS+DY fit, and comparing to the refitted distribution. We then use reweighting to determine the impact of recent high statistics lepton asymmetry data from the D0 experiment on the NNPDF2.0 parton set. We find that the D0 inclusive muon and electron data are perfectly compatible with the rest of the data included in the NNPDF2.0 analysis and impose additional constraints on the large-x d/u ratio. The more exclusive D0 electron datasets are however inconsistent both with the other datasets and among themselves, suggesting that here the experimental uncertainties have been underestimated.

==> sec-appA.tex <==
\section{Derivation of the Weights}
\label{sec:appA}

By the probability $P(f)$ for the PDF $f$ what we actually mean 
is the probability $P(f|K)$, where $K$ denotes all the data used in the determination and their associated errors, the values of parameters such as $\alpha_s$ and heavy quark masses used in the computation of the data 
expected from the PDF, and finally also the theoretical framework used (for example NLO QCD). If we then wish to extend the dataset by including new data $y$, the 
new probability $P_\new(f)$ is then $P(f|yK)$: besides $K$ we now also assume the new data $y$. 

The new probability is then determined from the old probability
using the sampling distribution $P(y|fK)$ and multiplicative rule for probabilities (often known as Bayes theorem):
\begin{equation}
P(AB|C)=P(A|BC)P(B|C) = P(B|AC)P(A|C),
\label{eq:Bayes}
\end{equation}
where $P(A|C)$ is the probabilities of $A$ given $C$, etc, and $AB$ denotes $A$ and $B$. Naively applying this result in the present case we have
\begin{equation}
P(f|yK)P(y|K) = P(y|fK)P(f|K),
\label{eq:Bayesmult}
\end{equation}
whence (replacing $P(f|K)$ with $\mathcal{P}(f|K)Df$, $P(f|yK)$ 
with $\mathcal{P}(f|yK)Df$)
\begin{equation}
\mathcal{P}(f|yK)= P(y|fK)\mathcal{P}(f|K)/P(y|K),
\label{eq:Bayespdf}
\end{equation}
Note that $\mathcal{P}(y|K)$ does not depend on the PDF $f$, and can thus be determining simply by insisting that $\mathcal{P}(f|yK)$ is properly normalized: we then find 
\begin{equation}
P(y|K)= \int P(y|fK)\mathcal{P}(f|K)Df,
\label{eq:marginalization}
\end{equation}
so
\begin{equation}
\mathcal{P}(f|yK)= P(y|fK)\mathcal{P}(f|K)\Big/\int P(y|fK)\mathcal{P}(f|K)Df,
\label{eq:Bayesdiscrete}
\end{equation}
where everything on the right hand side is now known.

This argument would work without problems if the data $y$ could only take discrete values. The difficulty in the present case is that our data are continuous, so rather than the probability $P(y|fK)$ we have to work with a multi-dimensional probability density $\mathcal{P}(y|fK)d^ny$, in a limit in which the volume element $d^ny$ goes to zero. Of course in this limit the probabilities $P(y|fK)$ and $P(y|K)$ also go to zero, and we find a ratio of two zeros in 
\eq{eq:Bayespdf}. The conditional probability $P(f|yK)$ is then only well defined if we specify carefully the way in which the limit is to be taken: probabilities conditional on sets of measure zero are ambiguous. Failure to specify the limiting process can result in contradictions (the Borel-Kolmogorov paradox \cite{Jaynes}).

Consider then the probability density for the data $y$. Assuming that the new experiments are not correlated with any
of the experiments used in the determination of the initial
probability density, the probability density of $y$ is then
given by \eq{eq:marginalization}:
\begin{equation}
  \mathcal{P}(y|K) = \int \mathcal{P}(y| fK)
  \mathcal{P}(f|K)\,Df = \smallfrac{1}{N}\sum_{k=1}^{N}
  \mathcal{P}(y|f_kK)
  \label{eq:dP},
\end{equation}
where in the second step we used \eq{eq:avg}. The density $\mathcal{P}(y|f K)$ gives the probability that the new data lie in an infinitesimal volume $d^n y$ centred at $y$ in the space of possible data given a particular choice of PDF $f$: it is often called the sampling distribution or (when considered as a function of $f$) the likelihood function. Assuming that the uncertainties in the data 
are purely Gaussian, 
\begin{equation}
  \mathcal{P}(y|fK)d^ny =(2\pi)^{-n/2}(\det \sigma_{ij})^{-1/2}
  e^{-\frac{1}{2}\chi^{2}(y,f)}d^ny,
  \label{eq:condP}
\end{equation}
where $\chi^{2}(y,f)$ is calculated using \eq{eq:chisq} (and of course using the assumptions $K$ in the computation of the predictions $y_i[f]$).

Since to compute $\mathcal{P}(y|fK)$ it is sufficient to compute $\chi^{2}(y,f)$, it is sufficient for our purposes to consider the probability density for the $\chi^2$ to the new dataset:
\begin{equation}
  \mathcal{P}(\chi^2|fK)d\chi^2 =
  2^{-n/2}(\Gamma(n/2))^{-1}(\chi^{2}(y,f))^{n/2-1}
  e^{-\frac{1}{2}\chi^{2}(y,f)}d\chi^2.
  \label{eq:condPcsq}
\end{equation}
This may be readily derived from \eq{eq:condP} by
diagonalising the covariance matrix and rescaling the data to a set
$\{Y_i\}$ of independent Gaussian variables each with unit
variance. Then $d^ny = (\det \sigma_{ij})^{1/2}d^nY$, and $\chi^2 =
\sum_{i=1}^n Y_i^2$.  Choosing $n$-dimensional spherical co-ordinates
in the space of data (with $\sqrt{\chi^2}$ as the radial co-ordinate,
and thus $y=y[f]$ as the origin), we may write $d^nY =
A_n\half(\chi^2)^{n/2-1}d\chi^2d^{n-1}\Omega$, where $d^{n-1}\Omega$
is the measure on the sphere and $A_n = 2\pi^{n/2}(\Gamma(n/2))^{-1}$
is the area of the unit sphere in $n$-dimensions. The probability
\eq{eq:condP} may thus be written
\begin{eqnarray}
  \mathcal{P}(y|fK)d^ny &=&(2\pi)^{-n/2}
  e^{-\frac{1}{2}\chi^{2}(y,f)}d^nY \nn \\ 
  &=& 2^{-n/2}(\Gamma(n/2))^{-1}(\chi^{2}(y,f))^{n/2-1}
  e^{-\frac{1}{2}\chi^{2}(y,f)} d\chi^2d^{n-1}\Omega.
  \label{eq:condPcsqderiv}
\end{eqnarray}
in agreement with \eq{eq:condPcsq} provided
\begin{equation}
  \mathcal{P}(y|fK)d^ny 
  = \mathcal{P}(\chi^2|fK)d\chi^2d^{n-1}\Omega.
  \label{eq:ytochirep}
\end{equation}
Again the probability density $\mathcal{P}(\chi^2|K)$ for the $\chi^2$
of the new dataset is obtained by averaging over replicas:
\begin{equation}
  \mathcal{P}(\chi^2|K) = \int \mathcal{P}(\chi^2|fK )
  \mathcal{P}(f|K)\,Df 
  = \smallfrac{1}{N}\sum_{k=1}^{N} \mathcal{P}(\chi^2|f_kK);
\label{eq:dPcsq}
\end{equation}
so combining \eq{eq:dP},\eq{eq:ytochirep}, and \eq{eq:dPcsq} 
\begin{equation}
  \mathcal{P}(y|K)d^ny 
  = \smallfrac{1}{N}\sum_{k=1}^{N} \mathcal{P}(\chi^2|f_kK)d\chi^2d^{n-1}\Omega 
  = \mathcal{P}(\chi^2|K)d\chi^2d^{n-1}\Omega, 
  \label{eq:ytochi}
\end{equation}
since both the volume factor $d^{n-1}\Omega$ and the interval
$d\chi^2$ are independent of the choice of replica, and may thus be
taken out of the sum.

The advantage of using $\mathcal{P}(\chi^2|fK)$ instead of $\mathcal{P}(y|fK)$ when evaluating \eq{eq:Bayespdf} is that $\mathcal{P}(\chi^2|fK)$ is only a one dimensional density, so the taking the limit is straightforward and unambiguous.
We may write \eq{eq:Bayespdf} as
\begin{equation}
\mathcal{P}(f|\chi^2K)Df\;\mathcal{P}(\chi^2|K)d\chi^2 
= \mathcal{P}(\chi^2|fK)d\chi^2\;\mathcal{P}(f|K)Df.
\label{eq:Bayescsq}
\end{equation}
The marginalization \eq{eq:dPcsq} follows directly on
integration over $f$, since if $\mathcal{P}(f|\chi^2)$ is correctly
normalized, $\int \mathcal{P}(f|\chi^2K)Df = 1$.  Now, cancelling the
$d\chi^2$ from either side of \eq{eq:Bayescsq} (since this is just a
pre-assigned interval),
\begin{equation}
 \mathcal{P}(f|\chi^2K)Df =
\frac{\mathcal{P}(\chi^2|fK)}{\mathcal{P}(\chi^2|K)}\mathcal{P}(f|K)Df.
\label{eq:newden}
\end{equation}
Multiplying on both sides by some observable $\O[f]$ and integrating
over the PDFs,
\begin{eqnarray}
\la\O\ra_{\new}&=&\int \O[f] \,
\mathcal{P}(f|\chi^2K)\,Df,\nn\\ &=&\int \O[f]
\,\frac{\mathcal{P}(\chi^2|fK)}{\mathcal{P}(\chi^2|K)}
\mathcal{P}(f|K)\,Df,\nn\\ 
&=&\frac{1}{N}\,\sum_{k=1}^{N}
\frac{\mathcal{P}(\chi^2|f_kK)}{\mathcal{P}(\chi^2|K)}
\mathcal{O}[f_k]\, ,
\label{eq:avgnewx}
\end{eqnarray}
where in the last line we used \eq{eq:avg}. This corresponds to the reweighting
\eq{eq:reweighting}
with weights
\begin{equation}
w_k = \frac{\mathcal{P}(\chi^2|f_kK)}{\mathcal{P}(\chi^2|K)}.
\label{eq:weightscsq}
\end{equation}
Combining \eq{eq:weightscsq} and
\eq{eq:condPcsq}, we obtain \eq{eq:weights},
with the normalization factor fixed as in \eq{eq:normcsq},
consistent with \eq{eq:weightscsq} and \eq{eq:dPcsq}.

Note that a further application of Bayes' theorem to \eq{eq:weightscsq} gives 
the alternative form
\begin{equation}
w_k = \frac{P(f_k|\chi^2K)}{P(f_k|K)}= N P(f_k|\chi^2K),
\label{eq:weightsprob}
\end{equation}
since because the replicas are uniformly distributed, $P(f_k|K)=1/N$. 
Thus $w_k/N$ is the probability of replica $f_k$ given the 
$\chi^2$ to the new data.

It is instructive to also derive the weights working directly with the 
probability density $\mathcal{P}(y|fK)$: using Bayes' theorem we may
write instead of \eq{eq:Bayescsq}
\begin{equation}
  \mathcal{P}(f|yK)Df\;\mathcal{P}(y|K)d^ny 
  = \mathcal{P}(y|fK)d^ny\;\mathcal{P}(f|K)Df.
  \label{eq:Bayesy}
\end{equation}
Again, the marginalization \eq{eq:dP} follows directly from
the normalization $\int \mathcal{P}(f|yK)Df = 1$.

Naively cancelling the volume factor
$d^ny$ from either side, and pursuing the same argument as before
yields:
\begin{eqnarray}
\la\O\ra_{\new}^G&=&\int \O[f] \, \mathcal{P}(f|yK)\,Df,\nn\\ 
&=&\int
\O[f] \,\frac{\mathcal{P}(y|fK)}{\mathcal{P}(y|K)}
\mathcal{P}(f|K)\,Df,\nn\\ 
&=&\frac{1}{N}\,\sum_{k=1}^{N}\frac{\mathcal{P}(y|f_kK)}{\mathcal{P}(y|K)}
\mathcal{O}[f_k]\, .
\label{eq:avgnewy}
\end{eqnarray}
This would then lead to the conclusion of Giele-Keller
\cite{Giele:1998gw} that the weights are proportional to
$\mathcal{P}(y|f_kK)/\mathcal{P}(y|K)$, and thus (using \eq{eq:condP})
are given by
\begin{equation}
w^G_k = \mathcal{N}_{G} e^{-\frac{1}{2}\chi^{2}(y,f_k)},
\label{eq:weightsgauss}
\end{equation}
with 
\begin{equation}
\mathcal{N}_{G}= N\Big/\sum_{k=1}^N e^{-\frac{1}{2}\chi^{2}(y,f_k)}.
\label{eq:normgauss}
\end{equation}
This result is clearly different from our previous result
\eq{eq:weightscsq}. We see explicitly that the densities $\mathcal{P}(f|\chi^2K)$ and
$\mathcal{P}(f|yK)$ are not the same, despite the fact that when the
data $y$ take a given value, the $\chi^2$ takes a corresponding value.
This is a nice example of the Borel-Kolmogorov paradox: 
the limits used to derive $\mathcal{P}(f|\chi^2K)$ and
$\mathcal{P}(f|yK)$ are different, and thus so are the results.

The probability density $\mathcal{P}(f|\chi^2K)$ is defined as the 
probability density for $f$ given that
the $\chi^2$ lies in the finite interval $[\chi^2,\chi^2+d\chi^2]$, in
the limit $d\chi^2\to 0$. In this case the conditioning variable spans
a one--dimensional manifold, and therefore there is no freedom in the
choice of the limiting procedure. The definition is unique, and thus
the argument which led to \eq{eq:weightscsq} was perfectly
satisfactory.

However the probability density $\mathcal{P}(f|yK)$ is defined as 
the probability density for $f$ given that $y$ lies in some 
volume $V_n$, in the limit $V_n\to 0$. In a multi-dimensional space 
such as this, the conditional
probability density $\mathcal{P}(f|yK)$ is ambiguous, since it depends
on the way the volume element $V_n$ is chosen. Different definitions
correspond to different physical settings. In the argument which led
us to \eq{eq:weightsgauss}, we implicitly assumed that $V_n$ was the
compact volume $d^ny$ centred on $y$, so that as $V_n\to 0$, the point
$y$ was uniquely selected. However there are many points in the 
space of data which have the same
$\chi^2$, and thus the same effect on $f$. If we want to include all
these points with equal weight when determining the conditional
probability density of $f$ given $y$, we need to sum over all the
compact volumes $d^ny$ that build the $(n-1)$-dimensional level surfaces of
$\chi^2(y,f)$ through the point $y$. Thus $V_n$ is a thin shell with
thickness $d\chi^2$, and hence its total volume is $V_n = A_n
d\chi^2$. The limit $V_n\to 0$ is then taken by letting $d\chi^2\to
0$. We thus write \eq{eq:Bayesy} as (using \eq{eq:ytochirep} and
\eq{eq:ytochi})
\begin{equation}
\mathcal{P}(f|yK) Df\;\mathcal{P}(\chi^2|K) A_n d\chi^2 
= \mathcal{P}(\chi^2|fK) A_n d\chi^2 \;\mathcal{P}(f|K)Df.
\label{eq:Bayesys}
\end{equation}
Cancelling the volume factor $A_n d\chi^2$, since this is independent
of $f$, this definition is now the same as \eq{eq:newden}, and thus
yields the correct weights \eq{eq:weights} in the limit $V_n\to 0$.


